Using LIP to Gloss Over Faces in Single-Stage Face Detection Networks

This work shows that it is possible to fool/attack recent state-of-the-art face detectors which are based on the single-stage networks. Successfully attacking face detectors could be a serious malware vulnerability when deploying a smart surveillance system utilizing face detectors. We show that existing adversarial perturbation methods are not effective to perform such an attack, especially when there are multiple faces in the input image. This is because the adversarial perturbation specifically generated for one face may disrupt the adversarial perturbation for another face. In this paper, we call this problem the Instance Perturbation Interference (IPI) problem. This IPI problem is addressed by studying the relationship between the deep neural network receptive field and the adversarial perturbation. As such, we propose the Localized Instance Perturbation (LIP) that uses adversarial perturbation constrained to the Effective Receptive Field (ERF) of a target to perform the attack. Experiment results show the LIP method massively outperforms existing adversarial perturbation generation methods -- often by a factor of 2 to 10.

==> Proposed_Work.tex <==
%------------------------------------------------------------------------
\section{Adversarial Examples for Scale-invariant Face Detection}


%------------------------------------------------------------------------
\subsection{Attack Targets and Goals}

\begin{figure}
\begin{center}
   \includegraphics[width=1\linewidth]{./figures/difficulty.jpg}
\end{center}
   \caption{The difficulties of different adversarial attack tasks. }
\label{fig:difficulty}
\end{figure}


%targets
For the adversarial attacks, the targets are different across different tasks.
We denote target as $t$ through this paper.
In image classification, the entire image is the target, whereas in semantic segmentation (or object detection), each pixel (or region proposal) is a target.
Let us assume an image has $K$ pixels (or $M$ proposals). The number of targets are $O(K)$ (or $O(M)$) in semantic segmentation (or object detection), while it is only $O(1)$ in image classification.
As the number of targets is much larger, the advesraial attacks in these two tasks are more difficult than in image classification~\cite{DAG}.

Also, because of the property of object detection that one object is associated with multiple region proposals, the generation of adversarial perturbations in object detection is more difficult than in segmentation.
If an object is associated with $K'$ pixels (or $M'$ proposlas), when $80\%$ of the pixels are successfully attacked, the attack rate is $80\%$. However, in object detection, if $99\%$ of the proposals are attacked successfully but with only $1\%$ proposals remained, the attack rate is $0$ as the remaining proposal will be recognised as a detection of the object.
As face detection is a special case of object detection, its difficulty in adversarial attacks seems to be the same as object detection. But 

%goals - targeted and untargeted
According to the goals of the adversarial attacks, the attacks can be categorised into \textit{non-targeted adversarial attack} and \textit{targeted adversarial attack}.
For non-targeted adversarial attack, the goal is to reduce the probability of the ground truth class $y^{true}$ of the given target $t$ and make the classification network predict any arbitrary class, whereas the goal of targeted adversarial attack it to ensure the classification network predict the target class $y^{target}$ for the target $t$.
Their object function can be summarised into the following formula:
\begin{equation*}
\min \quad \ell(f_\theta(x+\xi),t,y^{target})-\ell(f_\theta(x+\xi),t,y^{true}) \textrm{ .}
\end{equation*}


%face detection is multiple target and attack all classes
A multiclass classification problem can be considered as a combination of multiple binary classification problems.


In general, face detection is considered as a binary classification problem, which classifies a region as face or non-face.
In other words, $y^{target}=\{1,-1\}$.
However, in order to achieve scale-invariance, especially for small faces, the state-of-the-art scale-invariant face detectors~\cite{Tinyfaces,SSH,S3FD} divide face detection into multiple binary scale-specific classification problems and learn their loss functions jointly. 
Then the objective function is as follow:
\begin{equation*}
\min \quad \sum_{i=1}^S \ell_{s_{i}}(f_\theta(x+\xi),t,y^{target})  \textrm{ .}
\end{equation*}

It can be clearly see that the adversarial attacks for the scale-invariant face detectors is much more difficult than all the above-mentioned tasks. 
One face can be detected by multiple scale-specific classifiers.
Only when its proposals across all the scales are attacked successfully, the face can be removed.
We compare the difficulties of different tasks in Figure~\ref{fig:difficulty}.



% back to the details of our work
In this work, we aim to perform targeted adversarial attack in face detection. 
That is to remove the faces in the images.
In this work, we study the adversarial perturbations for the state-of-the-art face detector, HR~\cite{Tinyfaces}, which jointly learned 25 different scale-specific classifiers, \ie $S=25$.
First, we aim to perform targeted adversarial attack in face detection, which removes the true faces in the images. 
we set the target labels as $-1$ and then minimise the loss function:
\begin{equation}
\min \quad \sum_{i=1}^S \ell_{s_{i}}(f_\theta(x+\xi),t,-1)  \textrm{ .}
\end{equation}





%------------------------------------------------------------------------
\subsection{Effective Receptive Field}

Context is crucial in detecting small objects and recent deep learning based detectors extract features from the deeper layers to obtain the context information.
HR~\cite{Tinyfaces} extracted features from res4 to learn the context information.
Some recent works~\cite{ContextAwareSSD,S3FD} analysed the effective receptive field size for detecting small objects.
As mentioned above, the effective receptive field is a fraction of the theoretical receptive field which has effective impacts on the output.




%As mentioned above, due to the context information, one face can be significantly affected by the neighbouring faces.
%The Effective Receptive Field (ERF) is sufficient enough to attack.


%Need to mention the chain rule and initial value here?
Following~\cite{ERF}, we visualise the effective receptive field of a face by setting the initial value of the gradient of the center pixel of a face as 1, the gradients of the other pixels as 0.

The perturbation is based on the gradient so we want to analyse the effective receptive field?
Or to prove the effectiveness of ERF in another way, we analyse it in adversarial examples. After we crop it, it is still effective.

%------------------------------------------------------------------------
\subsection{ROI Perturbations Interference Problem}


Because convolution is translation invariant, the same image pixel receives the same responses (thus classification scores) irrespective to its relative position in the context.~\cite{instanceAwareSS}.


%1.only one fac
Let us consider an image that contains only one face (instance).
In this case, the original perturbations with respect to the entire image can produce a good mask for this instance as there is only one instance without interference from the other instances.

Next let's consider another situation that two faces are close to each other in an image.
There is overlap between the gradients of the two instances.


%------------------------------------------------------------------------
\section{Algorithm}




%------------------------------------------------------------------------
\subsection{Instance Aware Perturbations - Crop}

The above analysis motivates us to introduce the concept of \textit{instance aware perturbations} for adversarial perturbations.


We crop the perturbations according to the effective receptive field.
%-------------------------------------------------------------------------

\begin{figure}
\begin{center}
   \includegraphics[width=1\linewidth]{./figures/ERF.png}
\end{center}
   \caption{The Effective Receptive Field (ERF). }
\label{fig:ERF}
\end{figure}

%------------------------------------------------------------------------

%------------------------------------------------------------------------
\subsection{Process ROI separately}

compute the gradients of all active targets across all ROIs on the entire image only once and apply the ROI Pooling according to the ERF for each ROI. 

%------------------------------------------------------------------------
\begin{algorithm} % enter the algorithm environment
\caption{Two-stage Cascade Framework} % give the algorithm a caption
\label{alg1} % and a label for \ref{} commands later in the document
\begin{algorithmic}[1] % enter the algorithmic environment
    \REQUIRE Detector 1, detector 2
    \ENSURE A pair of cascade detectors
    \STATE Collect overlapping true and false positives\\ $\mathcal{T}_{o}=\mathcal{T}_{1} \cap \mathcal{T}_{2}, \mathcal{F}_{o}=\mathcal{F}_{1} \cap \mathcal{F}_{2}$
    \STATE Calculate the correlation and diversity \\$c^T_{2 \to 1}=\frac{|\mathcal{T}_{o}|}{|\mathcal{T}_{1}|}, d^F_{2 \to 1}=\frac{|\mathcal{F}_{o}|}{|\mathcal{F}_{1}|}$
    \WHILE{ $c^T_{2 \to 1} \approx 1$ and $d^F_{2 \to 1} \approx 1$}
        \IF{$t_1 < t_2$}
            \STATE cascade(detector 1, detector 2)
        \ELSE
            \STATE cascade(detector 2, detector 1)
        \ENDIF
    \ENDWHILE
\end{algorithmic}
\end{algorithm}
%------------------------------------------------------------------------

%------------------------------------------------------------------------
\subsection{Loss Max-Pooling - One Pixel Attack}

